The mass of our Milky Way

We perform an extensive review of the numerous studies and methods used to determine the total mass of the Milky Way. We group the various methods into seven broad classes, including: i) estimating Galactic escape velocity using high velocity objects; ii) measuring the rotation curve through terminal and circular velocities; iii) modeling halo stars, globular clusters and satellite galaxies with the Spherical Jeans equation and iv) with phase-space distribution functions; v) simulating and modeling the dynamics of stellar streams and their progenitors; vi) modeling the motion of the Milky Way, M31 and other distant satellites under the framework of Local Group timing argument; and vii) measurements made by linking the brightest Galactic satellites to their counterparts in simulations. For each class of methods, we introduce their theoretical and observational background, the method itself, the sample of available tracer objects, model assumptions, uncertainties, limits and the corresponding measurements that have been achieved in the past. Both the measured total masses within the radial range probed by tracer objects and the extrapolated virial masses are discussed and quoted. We also discuss the role of modern numerical simulations in terms of helping to validate model assumptions, understanding systematic uncertainties and calibrating the measurements. While measurements in the last two decades show a factor of two scatters, recent measurements using \textit{Gaia} DR2 data are approaching a higher precision. We end with a detailed discussion of future developments, especially as the size and quality of the observational data will increase tremendously with current and future surveys. In such cases, the systematic uncertainties will be dominant and thus will necessitate a much more rigorous testing and characterization of the various mass determination methods.

==> Makefile <==
MAIN=paper
OLD=old/paper
BIB=master.bib
STYLE=2017SCGE.cls aas_macros.sty picins.sty
#timestr=`date +%a-%d-%b`
timestr=`date -Idate`
#lineno.sty
TC=pdflatex

ifeq ($(TC), latex)
PC=dvipdf
else
PC=echo
endif

paper:
	$(TC) $(MAIN)
	bibtex $(MAIN)
	$(TC) $(MAIN)
	$(TC) $(MAIN)
	$(PC) $(MAIN)

diff:
	latexdiff $(OLD).tex $(MAIN).tex >diff.tex
	@make paper -e MAIN=diff
	@make clean -e MAIN=diff
	
tar: clean paper 
	mkdir tmp
	mkdir tmp/figures
	cp $(MAIN).tex $(MAIN).bbl $(BIB) $(STYLE) Makefile tmp/
	cp figures/*.pdf tmp/figures/
	cd tmp;	tar -czhf $(MAIN).$(timestr).tar.gz *; mv $(MAIN).$(timestr).tar.gz ../
	
clean:
	\rm -rf tmp
	\rm -f $(MAIN).aux $(MAIN).log $(MAIN).toc $(MAIN).blg $(MAIN).dvi $(MAIN).ps $(MAIN).out $(MAIN).bbl
	\rm -f diff.aux diff.log diff.toc diff.blg diff.dvi diff.ps diff.out diff.bbl

ultclean:
	\rm -rf tmp
	\rm -f *.aux *.log *.toc *.blg *.dvi *.ps *.out *.bbl *.backup $(MAIN).*.tar.gz $(MAIN).pdf
	\rm -f diff.pdf diff.tex


